Tracing Information Flows Between Ad Exchanges Using Retargeted Ads

Numerous surveys have shown that Web users are concerned about the loss of privacy associated with online tracking. Alarmingly, these surveys also reveal that people are also unaware of the amount of data sharing that occurs between ad exchanges, and thus underestimate the privacy risks associated with online tracking. In reality, the modern ad ecosystem is fueled by a flow of user data between trackers and ad exchanges. Although recent work has shown that ad exchanges routinely perform cookie matching with other exchanges, these studies are based on brittle heuristics that cannot detect all forms of information sharing, especially under adversarial conditions. In this study, we develop a methodology that is able to detect client- and server-side flows of information between arbitrary ad exchanges. Our key insight is to leverage retargeted ads as a tool for identifying information flows. Intuitively, our methodology works because it relies on the semantics of how exchanges serve ads, rather than focusing on specific cookie matching mechanisms. Using crawled data on 35,448 ad impressions, we show that our methodology can successfully categorize four different kinds of information sharing behavior between ad exchanges, including cases where existing heuristic methods fail. We conclude with a discussion of how our findings and methodologies can be leveraged to give users more control over what kind of ads they see and how their information is shared between ad exchanges.

==> chrome_tool.tex <==
\begin{figure}[t]
   \centering
   \includegraphics[height=6cm]
   {figures/dom-inclusion-tree-eps-converted-to.pdf}
   \caption{(a) DOM Tree, and (b) Inclusion Tree}
   \label{fig:dom-inclusion-tree}
\end{figure}

A website can include resources in an HTML document from any origin so long as the inclusion respects the same origin policy, its standard exceptions, or any additional policies due to the use of CSP, CORS, or other access control framework. Resources can be JavaScript code, image files, plugins such as Flash objects, or even other web pages loaded inside a frame.

A first approximation to understanding the inclusions of third-party content for a given web page is to process its DOM tree while the page loads. The DOM tree provides a natural structural representation of a web page that can be manipulated through a standard API, and can provide an indication of the chain of origins that lead to a resource inclusion. For instance, a web page $a$ could include another page $b$ within an \texttt{iframe} that then includes a script $c$. In this case, the inclusion relationship $a \rightarrow b \rightarrow c$ could be extracted directly from the DOM. Figure~\ref{fig:dom-inclusion-tree}(a) shows a sample DOM tree.

However, direct use of a web page's DOM tree is unsatisfactory because the DOM does not in fact reliably record the inclusion relationships between resources referenced by a page. This follows from the ability for JavaScript to manipulate the DOM at run-time; using the DOM API, JavaScript can add, modify, and remove DOM elements in an arbitrary fashion. As such, while the DOM is a faithful syntactic description of a web page \emph{at a given point in time}, it cannot be relied upon to extract relationships between included resources.

Instead, in this work we define an \emph{Inclusion Tree} abstraction extracted directly from the browser's resource loading code. Unlike a DOM tree, the inclusion tree precisely records the inclusion relationships between different resources in a web page that is invariant with respect to run-time DOM updates (under the assumption that all resource loads are observed). It also discards irrelevant portions of the DOM tree that do not reference remote content (e.g., \texttt{div}, \texttt{p}). In other words, inclusion trees represent the semantic inclusion structure of a web page, while DOM trees represent their syntactic structure. Figure~\ref{fig:dom-inclusion-tree}(b) shows the inclusion tree corresponding to the DOM tree in Figure~\ref{fig:dom-inclusion-tree}(a). As shown in Figure~\ref{fig:dom-inclusion-tree}(b), \texttt{c.org/flash.swf} has been added dynamically by \texttt{e.net/script.js} to the DOM tree.

For each resource in the inclusion tree, there is an \emph{inclusion chain}. An inclusion chain begins with the root resource $r_0$ (URL of web page). Each resource $r_{i+1}$ that is referenced by $r_i$ in the inclusion tree and that is loaded by the browser, inductively building a chain of resource inclusions $r_0 \rightarrow \dots \rightarrow r_i \rightarrow r_{i+1} \rightarrow \dots \rightarrow r_n$ for each resource $r_n$ included in the web page. For instance, as depicted in Figure~\ref{fig:dom-inclusion-tree}(b), there is an inclusion chain with length of 5 for resource \texttt{c.org/flash.swf}.



==> results.tex <==
\section{Additional Results}

\begin{table}[t]
\centering
\rowcolors{2}{gray!10}{white}
\begin{tabular}{r|l}
\textbf{Website} & \textbf{Retargeted Ads} \\
\hline
tumi.com & 176 \\
portero.com & 157 \\
personalizationmall.com & 132 \\
zzounds.com & 106 \\
sheplers.com & 104 \\
paulfredrick.com & 101 \\
thesak.com & 98 \\
luggagepros.com & 95 \\
6pm.com & 93 \\
soma.com & 92 \\
payless.com & 89 
\end{tabular}
\caption{Top 10 websites running campaigns}
\label{table:websites_retargeting}
\end{table}

\begin{table}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c}
\textbf{Retargeter} & \textbf{Platform} \\
\hline
criteo & googlesyndication  \\
googlesyndication & doubleclick  \\
steelhousemedia & googleadservices  \\
mythingsmedia & googletagservices  \\
2mdn & adnxs  \\
mediaforge & rubiconproject  \\
swansonvitamins & servedbyopenx  \\
scene7 & turner  \\
stewmac & openx  \\
thesak & mathtag  
\end{tabular}
\caption{Top domains}
\label{table:top_domains}
\end{table}


\break

\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c|c}
\textbf{Domain 1} & \textbf{Domain 2} & \textbf{Frequency} \\
\hline
google & googlesyndication & 5014 \\
doubleclick & googlesyndication & 5014 \\
googleadservices & googlesyndication & 4893 \\
google-analytics & googlesyndication & 3675 \\
googleapis & googlesyndication & 3573 \\
youtube & googlesyndication & 1771 \\
ytimg & googlesyndication & 1684 \\
googletagmanager & googlesyndication & 1413 \\
googleusercontent & googlesyndication & 1143 \\
googlecommerce & googlesyndication & 460 \\
doubleclick & 2mdn & 49 \\
google & 2mdn & 49 \\
google-analytics & 2mdn & 48 \\
googleadservices & 2mdn & 44 \\
googleusercontent & 2mdn & 10 \\
googleapis & 2mdn & 10 \\
googletagmanager & 2mdn & 7 \\
googletagmanager & doubleclick & 1
\end{tabular}
\caption{Domains responsible for reduction in Latent chains.}
\label{table:latent_analysis}
\end{table*}

\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c}
\textbf{Platform} & \textbf{Retargeter} \\
\hline
doubleclick (82) & criteo (178) \\
googlesyndication (75) & googlesyndication (113) \\
adnxs (40) & adnxs (17) \\
googleadservices (15) & yimg (12) \\
rubiconproject (13) & 2mdn (9) \\
pubmatic (7) & mathads (4) \\
atwola (4) & dotomi (4) \\
mathtag (4) & adtechus (3) \\
clickfuse (2) & mediaforge (1) \\
casalemedia (1) & mythingsmedia (1) \\
servedbyopenx (1) & images-amazon (1)
\end{tabular}
\caption{platform and retargeter in remaining Latent chains.}
\label{table:latent_remaining}
\end{table*}

\break

\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c|c}
\textbf{Domain 1} & \textbf{Domain 2} & \textbf{Frequency} \\
\hline
google & googlesyndication & 1926 \\
doubleclick & googlesyndication & 1926 \\
googleadservices & googlesyndication & 1869 \\
google-analytics & googlesyndication & 1605 \\
googleapis & googlesyndication & 1224 \\
googletagmanager & googlesyndication & 729 \\
youtube & googlesyndication & 379 \\
doubleclick & 2mdn & 371 \\
googleadservices & 2mdn & 368 \\
google-analytics & 2mdn & 365 \\
google & 2mdn & 353 \\
googleusercontent & googlesyndication & 348 \\
ytimg & googlesyndication & 347 \\
googleapis & 2mdn & 263 \\
googletagmanager & 2mdn & 257 \\
googlecommerce & googlesyndication & 240 \\
googleusercontent & 2mdn & 218 \\
yahoo & yimg & 32 \\
amazon-adsystem & images-amazon & 5 \\
youtube & 2mdn & 5 \\
ytimg & 2mdn & 5 \\
tellapart & tellaparts & 4 \\
doubleclick & googleusercontent & 2 \\
google-analytics & googleusercontent & 2 \\
googletagservices & googleusercontent & 2 \\
google & googleusercontent & 2 \\
googleadservices & googleusercontent & 2 \\
googlesyndication & googleusercontent & 2 \\
amazonaws & images-amazon & 1 \\
googletagservices & 2mdn & 1 \\
googlesyndication & 2mdn & 1
\end{tabular}
\caption{Domains responsible for reduction in Indirect chains.}
\label{table:indirect_analysis}
\end{table*}

\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c}
\textbf{Platform} & \textbf{Retargeter} \\
\hline
googlesyndication (59) & atlassbx (45) \\
atdmt (45) & mathads (42) \\
mathtag (45) & netmng (28) \\
rubiconproject (10) & adnxs (22) \\
doubleclick (6) & criteo (13) \\
adnxs (2) & googlesyndication (7) \\
dotomi (2) & mathtag (7)
\end{tabular}
\caption{platform and retargeter in remaining Indirect chains.}
\label{table:indirect_remaining}
\end{table*}

\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c|c}
\textbf{Done} & \textbf{Partial} & \textbf{None} \\
\hline
2mdn (2) & adlegend (4,1) & affinity (2) \\ 
adip (1) & adnxs (8,2) & atwola (7) \\ 
adsrvr (5) & adroll (3,2) & blogsmithmedia (1) \\ 
advertising (4) & adtechus (7,1) & emjcd (1) \\ 
amazon-adsystem (2) & clickfuse (1,1) & googleusercontent (1) \\ 
bidswitch (2) & googlesyndication (16,8) & images-amazon (1) \\ 
casalemedia (1) & mediaforge (4,1) & kinja-static (1) \\ 
connexity (1) & mediaplex (4,1) & mathads (2) \\ 
criteo (14) & pubmatic (3,1) & ssl-images-amazon (1) \\ 
dotomi (4) & steelhousemedia (3,1) & turner (1) \\ 
doubleclick (19) & tellapart (2,1) &  - \\ 
esm1 (2) &  - &  - \\ 
flashtalking (5) &  - &  - \\ 
googleadservices (1) &  - &  - \\ 
intermarkets (1) &  - &  - \\ 
lijit (1) &  - &  - \\ 
mathtag (4) &  - &  - \\ 
mythings (1) &  - &  - \\ 
mythingsmedia (1) &  - &  - \\ 
netmng (4) &  - &  - \\ 
openx (1) &  - &  - \\ 
openxenterprise (1) &  - &  - \\ 
quantserve (2) &  - &  - \\ 
rubiconproject (10) &  - &  - \\ 
scene7 (1) &  - &  - \\ 
servedbyopenx (1) &  - &  - \\ 
serving-sys (1) &  - &  - \\ 
taboola (1) &  - &  - \\ 
tubemogul (1) &  - &  - \\ 
tumri (1) &  - &  - \\ 
veruta (2) &  - &  - \\ 
yieldoptimizer (1) &  - &  - \\ 
yimg (2) &  - &  -
\end{tabular}
\caption{Platform matching in cookie validation}
\label{table:plat_validation}
\end{table*}


\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c|c}
\textbf{Done} & \textbf{Partial} & \textbf{None} \\
\hline
2mdn (2) & adlegend (4,1) & adacado (1) \\ 
adip (1) & adnxs (8,1) & affinity (2) \\ 
adsrvr (5) & adroll (3,2) & atwola (4) \\ 
adtechus (6) & clickfuse (1,1) & blogsmithmedia (0) \\ 
advertising (2) & domdex (1,1) & ebayimg (1) \\ 
amazon-adsystem (2) & googlesyndication (16,5) & emjcd (1) \\ 
bidswitch (2) & mediaforge (4,1) & googleusercontent (1) \\ 
casalemedia (1) & mediaplex (4,1) & images-amazon (1) \\ 
criteo (13) & pubmatic (3,1) & kinja-static (1) \\ 
dotomi (4) & steelhousemedia (3,2) & mathads (2) \\ 
doubleclick (17) & tellapart (2,1) & perfectaudience (1) \\ 
esm1 (3) &  - & ssl-images-amazon (1) \\ 
flashtalking (5) &  - & turner (1) \\ 
googleadservices (1) &  - &  - \\ 
lijit (1) &  - &  - \\ 
mathtag (5) &  - &  - \\ 
mythings (1) &  - &  - \\ 
mythingsmedia (1) &  - &  - \\ 
netmng (4) &  - &  - \\ 
openx (1) &  - &  - \\ 
quantserve (3) &  - &  - \\ 
rhythmxchange (1) &  - &  - \\ 
rubiconproject (9) &  - &  - \\ 
scene7 (1) &  - &  - \\ 
servedbyopenx (1) &  - &  - \\ 
serving-sys (1) &  - &  - \\ 
taboola (1) &  - &  - \\ 
tubemogul (1) &  - &  - \\ 
tumri (1) &  - &  - \\ 
veruta (3) &  - &  - \\ 
yieldoptimizer (1) &  - &  - \\ 
yimg (2) &  - &  -
\end{tabular}
\caption{Retargeter matching in cookie validation}
\label{table:ret_validation}
\end{table*}

Table~\ref{table:top_domains} shows the top retargeters and platforms by frequency (independent of each other).

\para{Latent Cases:} After clustering, the number of chains goes down from 5,362 to 343. Table~\ref{table:latent_analysis} shows the top domains responsible 
for this decrease in numbers. Table~\ref{table:latent_remaining} shows the platforms (predecessor) and retargeters in the remaining latent matching chains.  

\para{Indirect Cases:} After clustering, the number of chains goes down from 2,492 to 178. Table~\ref{table:indirect_analysis} shows the top domains responsible 
for this decrease in numbers. Table~\ref{table:indirect_remaining} shows the platforms (predecessor) and retargeters in the remaining indirect matching chains.

\para{Cookie Validation:} In total we have 112 cookie matching partners for forward cookie matching and 91 partners for backward cookie matching. In total there are 200 unique cookie matching partners. We try to validate these partners using the techniques used in prior works. Table~\ref{table:plat_validation} shows the platforms matches in these partner pairs where as Table~\ref{table:ret_validation} shows the retargeter matches.

Table~\ref{table:plat_validation_no_GS} and Table~\ref{table:ret_validation_no_GS} represents the same but here we assume that 'googlesyndication' is using 'doubleclick' cookie. This reduces the total partners to 173 and we validate 145 out of them.

\para{Cookie Mathing Partners:} See Table~\ref{table:cookie-partners-replica}.

\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c|c}
\textbf{Done} & \textbf{Partial} & \textbf{None} \\
\hline
2mdn (1) & adnxs (8,2) & affinity (2) \\ 
adip (1) & adroll (3,1) & atwola (7) \\ 
adlegend (1) & adtechus (7,1) & blogsmithmedia (1) \\ 
adsrvr (4) & clickfuse (1,1) & emjcd (1) \\ 
advertising (3) & doubleclick (26,1) & googleusercontent (1) \\ 
amazon-adsystem (2) & mediaplex (5,1) & images-amazon (1) \\ 
bidswitch (2) & pubmatic (3,1) & kinja-static (1) \\ 
casalemedia (1) &  - & mathads (2) \\ 
connexity (1) &  - & ssl-images-amazon (1) \\ 
criteo (13) &  - & turner (1) \\ 
dotomi (3) &  - &  - \\ 
esm1 (2) &  - &  - \\ 
flashtalking (4) &  - &  - \\ 
googleadservices (1) &  - &  - \\ 
intermarkets (1) &  - &  - \\ 
lijit (1) &  - &  - \\ 
mathtag (4) &  - &  - \\ 
mediaforge (4) &  - &  - \\ 
mythings (1) &  - &  - \\ 
mythingsmedia (1) &  - &  - \\ 
netmng (3) &  - &  - \\ 
openx (1) &  - &  - \\ 
openxenterprise (1) &  - &  - \\ 
quantserve (2) &  - &  - \\ 
rubiconproject (10) &  - &  - \\ 
scene7 (1) &  - &  - \\ 
servedbyopenx (1) &  - &  - \\ 
serving-sys (1) &  - &  - \\ 
steelhousemedia (2) &  - &  - \\ 
taboola (1) &  - &  - \\ 
tellapart (2) &  - &  - \\ 
tubemogul (1) &  - &  - \\ 
tumri (1) &  - &  - \\ 
veruta (2) &  - &  - \\ 
yieldoptimizer (1) &  - &  - \\ 
yimg (2) &  - &  -
\end{tabular}
\caption{Platform matching in cookie validation without googlesyndication}
\label{table:plat_validation_no_GS}
\end{table*}


\begin{table*}[t]
\rowcolors{2}{gray!10}{white}
\centering
\begin{tabular}{c|c|c}
\textbf{Done} & \textbf{Partial} & \textbf{None} \\
\hline
2mdn (1) & adnxs (8,1) & adacado (1) \\ 
adip (1) & adroll (3,1) & affinity (2) \\ 
adlegend (4) & clickfuse (1,1) & atwola (4) \\ 
adsrvr (4) & pubmatic (3,1) & blogsmithmedia (0) \\ 
adtechus (6) & steelhousemedia (3,1) & ebayimg (1) \\ 
advertising (1) &  - & emjcd (1) \\ 
amazon-adsystem (2) &  - & googleusercontent (1) \\ 
bidswitch (2) &  - & images-amazon (1) \\ 
casalemedia (1) &  - & kinja-static (1) \\ 
criteo (12) &  - & mathads (2) \\ 
domdex (2) &  - & perfectaudience (1) \\ 
dotomi (3) &  - & ssl-images-amazon (1) \\ 
doubleclick (23) &  - & turner (1) \\ 
esm1 (2) &  - &  - \\ 
flashtalking (4) &  - &  - \\ 
googleadservices (1) &  - &  - \\ 
lijit (1) &  - &  - \\ 
mathtag (5) &  - &  - \\ 
mediaforge (4) &  - &  - \\ 
mediaplex (5) &  - &  - \\ 
mythings (1) &  - &  - \\ 
mythingsmedia (1) &  - &  - \\ 
netmng (3) &  - &  - \\ 
openx (1) &  - &  - \\ 
quantserve (2) &  - &  - \\ 
rhythmxchange (1) &  - &  - \\ 
rubiconproject (9) &  - &  - \\ 
scene7 (1) &  - &  - \\ 
servedbyopenx (1) &  - &  - \\ 
serving-sys (1) &  - &  - \\ 
taboola (1) &  - &  - \\ 
tellapart (1) &  - &  - \\ 
tubemogul (1) &  - &  - \\ 
tumri (1) &  - &  - \\ 
veruta (2) &  - &  - \\ 
yieldoptimizer (1) &  - &  - \\ 
yimg (2) &  - &  -
\end{tabular}
\caption{Retargeter matching in cookie validation without googlesyndication}
\label{table:ret_validation_no_GS}
\end{table*}


